Non-adaptive Combinatorial Quantitative Group Testing with Adversarially Perturbed Measurements

In this paper, combinatorial quantitative group testing (QGT) with noisy measurements is studied. The goal of QGT is to detect defective items from a data set of size $n$ with counting measurements, each of which counts the number of defects in a selected pool of items. While most literatures consider either probabilistic QGT with random noise or combinatorial QGT with noiseless measurements, our focus is on the combinatorial QGT with noisy measurements that might be adversarially perturbed by additive bounded noises. Since perfect detection is impossible, a partial detection criterion is adopted. With the adversarial noise being bounded by $d_n = \Theta(n^\delta)$ and the detection criterion being to ensure no more than $k_n = \Theta(n^\kappa)$ errors can be made, our goal is to characterize the fundamental limit on the number of measurement, termed \emph{pooling complexity}, as well as provide explicit construction of measurement plans with optimal pooling complexity and efficient decoding algorithms. We first show that the fundamental limit is $\frac{1}{1-2\delta}\frac{n}{\log n}$ to within a constant factor not depending on $(n,\kappa,\delta)$ for the non-adaptive setting when $0<2\delta\leq \kappa <1$, sharpening the previous result by Chen and Wang [2]. We also provide an explicit construction of a non-adaptive deterministic measurement plan with $\frac{1}{1-2\delta}\frac{n}{\log_{2} n}$ pooling complexity up to a constant factor, matching the fundamental limit, with decoding complexity being $o(n^{1+\rho})$ for all $\rho > 0$, nearly linear in $n$, the size of the data set.

==> old.tex <==
As for the construction of SCQGT algorithms, although our construction is sub-optimal in pooling complexity ($o(n^{\lambda+\rho})$ for all $\rho > 0$), it can be combined with the above-mentioned sub-optimal measurement plan for CQGT to yield a non-adaptive measurement plan with pooling complexity being $\frac{1}{1-2\delta}\frac{n}{\log_{2} n}$ to within a constant factor (optimal in the leading coefficient) for the CQGT problem. Furthermore, it is the first deterministic and non-adaptive construction that can handle severe infinity-norm noise within outcomes of every counting measurement. Moreover, its high-level idea, called the \emph{embedding method}, can serve as a general principle to construct deterministic and non-adaptive pooling algorithms in other problems with a sparse structure such as compressed sensing, group testing, quantitative group testing, and others. Unlike adaptive and random cases, there are no general principles to construct deterministic and non-adaptive pooling algorithms in these problems. 

For adaptive case, one can follow the principle of generalized binary splitting algorithms\cite{generalized-binary-splitting}, as in noisy adaptive compressed sensing\cite{CS-adaptive}, noisy adaptive group testing\cite{GT-adaptive}, and noisy quantitative group testing\cite{QGT-adaptive} to sequentially locate defective items. For constructing random and non-adaptive design, there also exist general principles such as sparse-graph code based construction in noisy compressed sensing\cite{CS-sparse-graph-code}, noisy group testing\cite{GT-sparse-graph-code}, and quantitative group testing\cite{QGT-sparse-graph-code} or leverage randomness to equivalently perform adaptive search non-adaptively\cite{GT-adaptive-to-non-adaptive-by-randomness}. However, these principles cannot extend to construct deterministic and non-adaptive pooling algorithms. Existing deterministic and non-adaptive constructions in group testing\cite{GT-non-adaptive-non-random} and compressed sensing\cite{CS-deterministic-survey} are problem-specific. They all use algebra-based methods (typically from error-correcting codes) and are consequently hard to extend to different noise models. Once the type of query and noise model changes, it induces a brain-new combinatorial problem, and one needs to solve it all over again.

On the other hand, our embedding idea provides a high-level principle to construct deterministic and non-adaptive algorithms in general sparse-related problems. It decomposes the whole problem into two steps. First, we consider the same problem but without a sparse structure. Typically, the difficulty would dramatically reduce. For example, a noisy, compressed sensing problem without sparse constraints reduce to a linear regression problem. Therefore we can get deterministic and non-adaptive constructions $\mb{M}$ more easily. Second, we tried to embed many small-versioned $\mb{M}$ into the final pooling matrix $\mb{M}_{s}$ for the original problem with sparse constraints so that whatever the support set of the hidden data is, the corresponding column-submatrix of $\mb{M}_{s}$ always contain a sub matrix similar to $\mb{M}$. Consequently $\mb{M}_{s}$ is a good pooling matrix for the original problem with sparse constraints. In this work, we follow this two-step framework to solve the noisy SCQGT problem. First, we solve the case without sparse constraints, which is reduced to the noisy CQGT problem. Then, we embed our solution matrix for CQGT into the constructed pooling matrix for SCQGT by leveraging a specific combinatorial structure called lossless unbalanced bipartite expanders \cite{Ta-ShmaUmans_07, expander_construction}. While the existence of unbalanced bipartite expanders with the optimal parameters can be proved via probabilistic methods, the explicit construction that achieves the optimal parameters remain open to the best of our knowledge. Fortunately, the near-optimal construction in Guruswami \textit{et al.} \cite{expander_construction} suffices to meet our need.  As a result, we provide an explicit construction of a non-adaptive measurement plan for the SCQGT problem with sub-optimal pooling complexity ($o(n^{\lambda+\rho})$ for all $\rho > 0$). If an optimal construction of unbalanced bipartite expanders is given, together with a little adjustment, our pooling complexity can be improved to $n^{\lambda}\log\lp n\rp\log\lp\log\lp n\rp\rp$. 

\iffalse
Our proposed construction has the several benefits in practical applications.
\begin{itemize}
    \item We provide an efficient decoding algorithm with computational complexity near linear in $n$ ($o\lp n^{1+\rho}\rp$ for all $\rho>0$).
    \item It is non-adaptive. There does not exist dependency between pools. Hence, all pooling can be carried out parallelly to save time of the overall measuring process.
    \item It is deterministic. Therefore we can leverage its fixed structure to save time and space resources in the decoding process. Moreover, it provides combinatorial guarantee.
\end{itemize}
\fi

The main idea behind our construction, called an \emph{embedding approach}, provides a high-level principle to construct deterministic and non-adaptive algorithms in general sparsity-related problems. It decomposes the whole problem into two steps. First, we consider the same problem but without a sparse structure. Typically, the difficulty would dramatically reduce. For example, a noisy, compressed sensing problem without sparse constraints reduce to a linear regression problem. Therefore we can get deterministic and non-adaptive constructions $\mb{M}$ more easily. Second, we tried to embed many small-versioned $\mb{M}$ into the final pooling matrix $\mb{M}_{s}$ for the original problem with sparse constraints so that whatever the support set of the hidden data is, the corresponding column-submatrix of $\mb{M}_{s}$ always contain a sub matrix similar to $\mb{M}$. Consequently $\mb{M}_{s}$ is a good pooling matrix for the original problem with sparse constraints. In this work, we follow this two-step framework to solve the noisy SCQGT problem. First, we solve the case without sparse constraints, which is reduced to the noisy CQGT problem. Then, we embed our solution matrix for CQGT into the constructed pooling matrix for SCQGT by leveraging a specific combinatorial structure called lossless unbalanced bipartite expanders \cite{Ta-ShmaUmans_07, expander_construction}. While the existence of unbalanced bipartite expanders with the optimal parameters can be proved via probabilistic methods, the explicit construction that achieves the optimal parameters remain open to the best of our knowledge. Fortunately, the near-optimal construction in Guruswami \textit{et al.} \cite{expander_construction} suffices to meet our need.  As a result, we provide an explicit construction of a non-adaptive measurement plan for the SCQGT problem with sub-optimal pooling complexity ($o(n^{\lambda+\rho})$ for all $\rho > 0$). If an optimal construction of unbalanced bipartite expanders is given, together with a little adjustment, our pooling complexity can be improved to $n^{\lambda}\log\lp n\rp\log\lp\log\lp n\rp\rp$. 

\iffalse
It is worth noting that in many real applications, deterministic non-adaptive measurement plans are more favorable. For the deterministic part, since deterministic constructions are more structured than probabilistic ones, it can leverage its 2 specific structures to lower the decoding complexity (time and apace). For the adeptness part, a highly adaptive pooling algorithm can only make a query until the results of previous queries are revealed. Unfortunately, in many real applications such as bioinformatics, each query takes time, and hence the overall waiting time is too long and not practical. In contrast, for non-adaptive pooling algorithms, there doesn’t exist dependency between pools. Hence, all queries can be carried out in parallel to save a huge amount of time and make the algorithm practical. In this work, all measurement plans we proposed are deterministic and non-adaptive, which makes our results more practical than previous literature. For efficient decoding, the complexity is dominated by the SCQGT part, where we leverage the Sparse Matching Pursuit algorithm in \cite{expander_algorithm}, and the overall decoding complexity is 
%$O\lp n\frac{\lambda\lp\lambda-2\delta\rp \log(n)^{3}}{\epsilon}2^{\sqrt{\frac{\lambda \log(n) \log\lp \frac{\lambda \log(n)^{2}}{\epsilon}\rp }{3}}}\rp$, which is 
$o(n^{1+\rho})$ for all $\rho > 0$, nearly linear in $n$. 
Note that in \cite{expander_algorithm}, the Sparse Matching Pursuit algorithm is proposed for recovering sparse real-valued vector from measurements generated by binary sensing matrices, and hence it can be used to recover sparse binary vector.

For the third contribution, the high-level intuition behind is structure embedding. To do this, we require 
\begin{enumerate}
    \item A good construction that can distinguish all possible data under noise even if it suffers from a certain degree of corruption.
    \item An embedding method that will combine with the above-mentioned construction to make sure all concerned data pairs can be separated under noise.
\end{enumerate}
For example, in our construction for the Sparse Combinatorial Quantitative Group Testing problem(SCQGT), we have
\begin{enumerate}
    \item Hadamard matrix serves as a good pooling matrix to distinguish all data vectors under infinity norm noise.
    \item An embedding method utilizes an unbalanced bipartite expander graph to embed many small Hadamard-like structures into our final pooling matrix.
\end{enumerate}
As a result, for all sufficient sparse vectors, those column vectors in our constructed pooling matrix corresponding to its support would contain a Hadamard-like submatrix. Consequently, our pooling matrix can distinguish all concerned data pairs of sufficiently sparse vectors.
\fi

By the linearity of the measuring process, distinguishing two binary data vectors $\bm{x}_{1},\bm{x}_{2}$ is equivalent to covering their difference vector $\bm{d}:=\bm{x}_{1}-\bm{x}_{2}\in\{0,\pm 1\}^{n}$. We say a pooling matrix $\mb{P}$ covers a difference vector $\bm{d}$ if $\lnorm \mb{P}\bm{d}\rnorm_{\infty}\geq 2n^{\delta}$, which implies that we can distinguish $\bm{x}_{1},\bm{x}_{2}$ even each measurement outcome is perturbed by noise with strength smaller than $n^{\delta}$.

sparse difference vector, $n^{\kappa}\leq\lnorm \bm{d}\rnorm_{0}\leq 2n^{\lambda},\kappa\leq \lambda <1$

 It has two steps. 
\begin{enumerate}
    \item First, we figure out how to do this without sparse structure, constructing a $2n^{\lambda}$ by $2n^{\lambda}$ matrix $\mb{H}$ with property that $\forall \bm{d}\in\{0,\pm 1\}^{2n^{\lambda}}$ and $n^{\kappa}\leq\lnorm \bm{d}\rnorm_{0}\leq 2n^{\lambda}$ 
    \begin{equation*}
        \lnorm \mb{H}\bm{d}\rnorm_{\infty}\geq 2n^{\delta}.    
    \end{equation*}
    \item Second, we design an embedding method to embed this matrix $\mb{H}$ into our final $n^{\lambda}\log(n)$ by $n$ detecting matrix $\mb{P}$. Where embedding means that for all submatrices $\mb{P}_{2n^{\lambda}}$ composed by $2n^{\lambda}$ columns of $\mb{P}$, there always exists a submatrix $\mb{H}_{p}$ composed by $2n^{\lambda}$ rows of $\mb{P}_{2n^{\lambda}}$ such that after certain row and column permutations $\sigma_{r},\sigma_{c}$, $\sigma_{r}(\sigma_{c}(\mb{H}_{p}))=\mb{H}$.
\end{enumerate}
If we complete these two steps, then by the definition of $\mb{H},\mb{P}$, we can solve the problem. However, the embedding criteria in step 2 is difficult to reach. Since we need to make sure that all $\tbinom{n}{2n^{\lambda}}$ submatrices $\mb{P}_{2n^{\lambda}}$ satisfy this criterion. The key idea in our embedding method is that we can trade difficulty of dealing with sparse structures in step 2 with designing a robust detecting matrix $\mb{H}$. If we carefully design a robust detecting matrix $\mb{H}$ in step 1 such that it can do its job even with certain perturbation, then we can largely relax our embedding criteria in step 2. We only need $\sigma_{r}(\sigma_{c}(\mb{H}_{p}))$ looks roughly like $\mb{H}$ instead of exactly equal to $\mb{H}$. Once the difference between $\sigma_{r}(\sigma_{c}(\mb{H}_{p}))$ and $\mb{H}$ does not exceed the robustness level of $\mb{H}$, the whole job can still be done. This framework is valuable because, in many cases, designing robust detecting matrices without sparse constraints is easier than directly dealing with sparse structures.





where $\lp \bm{x}-\bm{x}'\rp_{fold}^{i}$ is defined as a $M\times 1$ vector such that 
\begin{equation*}
    \lp \bm{x}-\bm{x}'\rp_{fold}^{i}(j):=\sum_{z:z\text{'th column at }\mb{B}_{i}\text{ has it's non zero element at }j\text{-th place}}\lp x-x'\rp(z)
\end{equation*}
and 
